The Identification of Asymmetric Barred Galaxies in Illustris TNG-50

Most barred galaxies exhibit symmetric structures. However, recent studies have shown that a subset of barred galaxies exhibit lopsided morphologies. To quantify their occurrence and investigate their physical origins, we analyze barred galaxies in the IllustrisTNG TNG50 simulation. We select 519 clearly barred galaxies in their stellar mass maps out of 770 barred galaxies from the TNG50-1 catalog. We classify the bar morphologies into four subgroups - `Lopsided', `Perturbed', `Symmetric', and `Indeterminate' - and perform a comparative analysis of their physical properties. We find that galaxies hosting asymmetric bars (`Lopsided' and `Perturbed') tend to have higher gas densities around the bar region, enhanced star formation activity, and more recent bar-formation epochs than galaxies with symmetric bars. However, the factor that most consistently distinguishes the four subgroups is the stellar mass distribution of the host galaxy, and there appears to be no physical correlation with bar size. These findings suggest that asymmetric bars form preferentially in less massive galaxies and may evolve into symmetric bars over time through secular processes. However, this conclusion should be considered with caution, as the fraction of asymmetric bars in the TNG50 simulation is systematically higher than that observed in the local universe.

==> jkas-Asymmetric_bar <==
\begin{thebibliography}{}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\href{#1}{#1}}
\providecommand{\dodoi}[1]{doi:~\href{http://doi.org/#1}{\nolinkurl{#1}}}
\providecommand{\doeprint}[1]{\href{http://ascl.net/#1}{\nolinkurl{http://ascl.net/#1}}}
\providecommand{\doarXiv}[1]{\href{https://arxiv.org/abs/#1}{\nolinkurl{https://arxiv.org/abs/#1}}}
\providecommand{\dodoilink}[2]{\href{http://doi.org/#1}{#2}}
\providecommand{\doadslink}[2]{\href{#1}{#2}}

\bibitem[{{Aguerri} {et~al.}(2009){Aguerri}, {M{\'e}ndez-Abreu}, \& {Corsini}}]{aguerri_2009}
{Aguerri}, J.~A.~L., {M{\'e}ndez-Abreu}, J., \& {Corsini}, E.~M. 2009, \aap, 495, 491

\bibitem[{{Alonso} {et~al.}(2018){Alonso}, {Coldwell}, {Duplancic}, {Mesa}, \& {Lambas}}]{alonso_2018}
{Alonso}, S., {Coldwell}, G., {Duplancic}, F., {Mesa}, V., \& {Lambas}, D.~G. 2018, \aap, 618, A149

\bibitem[{{Athanassoula}(1992)}]{athanassoula_1992a}
{Athanassoula}, E. 1992, \mnras, 259, 328

\bibitem[{{Athanassoula}(1996)}]{athanassoula_1996}
{Athanassoula}, E. 1996, in Astronomical Society of the Pacific Conference Series, Vol.~91, IAU Colloquium 157: Barred Galaxies, ed. R.~{Buta}, D.~A. {Crocker}, \& B.~G. {Elmegreen}, 309

\bibitem[{{Athanassoula}(2005)}]{athanassoula_2005}
{Athanassoula}, E. 2005, \mnras, 358, 1477

\bibitem[{{Athanassoula} {et~al.}(2013){Athanassoula}, {Machado}, \& {Rodionov}}]{athanassoula_2013}
{Athanassoula}, E., {Machado}, R. E.~G., \& {Rodionov}, S.~A. 2013, \mnras, 429, 1949

\bibitem[{{Athanassoula} {et~al.}(2009){Athanassoula}, {Romero-G{\'o}mez}, {Bosma}, \& {Masdemont}}]{athanassoula_2009}
{Athanassoula}, E., {Romero-G{\'o}mez}, M., {Bosma}, A., \& {Masdemont}, J.~J. 2009, \mnras, 400, 1706

\bibitem[{{Baes} {et~al.}(2011){Baes}, {Verstappen}, {De Looze}, {Fritz}, {Saftly}, {Vidal P{\'e}rez}, {Stalevski}, \& {Valcke}}]{baes_2011}
{Baes}, M., {Verstappen}, J., {De Looze}, I., {et~al.} 2011, \apjs, 196, 22

\bibitem[{{Bekki}(2009)}]{bekki_2009}
{Bekki}, K. 2009, \mnras, 393, L60

\bibitem[{{Berentzen} {et~al.}(2003){Berentzen}, {Athanassoula}, {Heller}, \& {Fricke}}]{berentzen_2003}
{Berentzen}, I., {Athanassoula}, E., {Heller}, C.~H., \& {Fricke}, K.~J. 2003, \mnras, 341, 343

\bibitem[{{Berentzen} {et~al.}(2007){Berentzen}, {Shlosman}, {Martinez-Valpuesta}, \& {Heller}}]{berentzen_2007}
{Berentzen}, I., {Shlosman}, I., {Martinez-Valpuesta}, I., \& {Heller}, C.~H. 2007, \apj, 666, 189

\bibitem[{{Bournaud} {et~al.}(2005){Bournaud}, {Combes}, \& {Semelin}}]{bournaud_2005}
{Bournaud}, F., {Combes}, F., \& {Semelin}, B. 2005, \mnras, 364, L18

\bibitem[{Bournaud {et~al.}(2007)Bournaud, Elmegreen, \& Elmegreen}]{bournaud_2007}
Bournaud, F., Elmegreen, B.~G., \& Elmegreen, D.~M. 2007, The Astrophysical Journal, 670, 237

\bibitem[{{Buta} {et~al.}(2005){Buta}, {Vasylyev}, {Salo}, \& {Laurikainen}}]{buta_2005}
{Buta}, R., {Vasylyev}, S., {Salo}, H., \& {Laurikainen}, E. 2005, \aj, 130, 506

\bibitem[{{Buta}(2017)}]{buta_2017b}
{Buta}, R.~J. 2017, \mnras, 470, 3819

\bibitem[{{Buta} {et~al.}(2009){Buta}, {Knapen}, {Elmegreen}, {Salo}, {Laurikainen}, {Elmegreen}, {Puerari}, \& {Block}}]{buta_2009a}
{Buta}, R.~J., {Knapen}, J.~H., {Elmegreen}, B.~G., {et~al.} 2009, \aj, 137, 4487

\bibitem[{{Buta} {et~al.}(2015){Buta}, {Sheth}, {Athanassoula}, {Bosma}, {Knapen}, {Laurikainen}, {Salo}, {Elmegreen}, {Ho}, {Zaritsky}, {Courtois}, {Hinz}, {Mu{\~n}oz-Mateos}, {Kim}, {Regan}, {Gadotti}, {Gil de Paz}, {Laine}, {Men{\'e}ndez-Delmestre}, {Comer{\'o}n}, {Erroz Ferrer}, {Seibert}, {Mizusawa}, {Holwerda}, \& {Madore}}]{buta_2015}
{Buta}, R.~J., {Sheth}, K., {Athanassoula}, E., {et~al.} 2015, \apjs, 217, 32

\bibitem[{{Camps} \& {Baes}(2015)}]{camps_2015}
{Camps}, P., \& {Baes}, M. 2015, Astronomy and Computing, 9, 20

\bibitem[{{Ceverino} {et~al.}(2010){Ceverino}, {Dekel}, \& {Bournaud}}]{ceverino_2010}
{Ceverino}, D., {Dekel}, A., \& {Bournaud}, F. 2010, \mnras, 404, 2151

\bibitem[{{Cheung} {et~al.}(2013){Cheung}, {Athanassoula}, {Masters}, {Nichol}, {Bosma}, {Bell}, {Faber}, {Koo}, {Lintott}, {Melvin}, {Schawinski}, {Skibba}, \& {Willett}}]{cheung_2013}
{Cheung}, E., {Athanassoula}, E., {Masters}, K.~L., {et~al.} 2013, \apj, 779, 162

\bibitem[{{Cheung} {et~al.}(2015){Cheung}, {Trump}, {Athanassoula}, {Bamford}, {Bell}, {Bosma}, {Cardamone}, {Casteels}, {Faber}, {Fang}, {Fortson}, {Kocevski}, {Koo}, {Laine}, {Lintott}, {Masters}, {Melvin}, {Nichol}, {Schawinski}, {Simmons}, {Smethurst}, \& {Willett}}]{cheung_2015}
{Cheung}, E., {Trump}, J.~R., {Athanassoula}, E., {et~al.} 2015, \mnras, 447, 506

\bibitem[{{Cisternas} {et~al.}(2015){Cisternas}, {Sheth}, {Salvato}, {Knapen}, {Civano}, \& {Santini}}]{cisternas_2015}
{Cisternas}, M., {Sheth}, K., {Salvato}, M., {et~al.} 2015, \apj, 802, 137

\bibitem[{{Col{\'{\i}}n} \& {Athanassoula}(1989)}]{colin_1989}
{Col{\'{\i}}n}, J., \& {Athanassoula}, E. 1989, Astronomy and Astrophysics, 214, 99

\bibitem[{{Conselice}(2014)}]{conselice_2014}
{Conselice}, C.~J. 2014, \araa, 52, 291

\bibitem[{{Cuomo} {et~al.}(2022){Cuomo}, {Corsini}, {Morelli}, {Aguerri}, {Lee}, {Coccato}, {Pizzella}, {Buttitta}, \& {Gasparri}}]{cuomo_2022}
{Cuomo}, V., {Corsini}, E.~M., {Morelli}, L., {et~al.} 2022, \mnras, 516, L24

\bibitem[{{de Lorenzo-C{\'a}ceres} {et~al.}(2019){de Lorenzo-C{\'a}ceres}, {S{\'a}nchez-Bl{\'a}zquez}, {M{\'e}ndez-Abreu}, {Gadotti}, {Falc{\'o}n-Barroso}, {Mart{\'\i}nez-Valpuesta}, {Coelho}, {Fragkoudi}, {Husemann}, {Leaman}, {P{\'e}rez}, {Querejeta}, {Seidel}, \& {van de Ven}}]{delorenzo_2019}
{de Lorenzo-C{\'a}ceres}, A., {S{\'a}nchez-Bl{\'a}zquez}, P., {M{\'e}ndez-Abreu}, J., {et~al.} 2019, \mnras, 484, 5296

\bibitem[{{de S{\'a}-Freitas} {et~al.}(2023){de S{\'a}-Freitas}, {Fragkoudi}, {Gadotti}, {Falc{\'o}n-Barroso}, {Bittner}, {S{\'a}nchez-Bl{\'a}zquez}, {van de Ven}, {Bieri}, {Coccato}, {Coelho}, {Fahrion}, {Gon{\c{c}}alves}, {Kim}, {de Lorenzo-C{\'a}ceres}, {Martig}, {Mart{\'\i}n-Navarro}, {Mendez-Abreu}, {Neumann}, \& {Querejeta}}]{desafreitas_2023}
{de S{\'a}-Freitas}, C., {Fragkoudi}, F., {Gadotti}, D.~A., {et~al.} 2023, \aap, 671, A8

\bibitem[{{de Swardt} {et~al.}(2015){de Swardt}, {Sheth}, {Kim}, {Pardy}, {D'Onghia}, {Wilcots}, {Hinz}, {Mu{\~n}oz-Mateos}, {Regan}, {Athanassoula}, {Bosma}, {Buta}, {Cisternas}, {Comer{\'o}n}, {Gadotti}, {Gil de Paz}, {Jarrett}, {Elmegreen}, {Erroz-Ferrer}, {Ho}, {Knapen}, {Laine}, {Laurikainen}, {Madore}, {Meidt}, {Men{\'e}ndez-Delmestre}, {Peng}, {Salo}, {Schinnerer}, \& {Zaritsky}}]{deswardt_2015}
{de Swardt}, B., {Sheth}, K., {Kim}, T., {et~al.} 2015, \apj, 808, 90

\bibitem[{{Debattista} {et~al.}(2006){Debattista}, {Mayer}, {Carollo}, {Moore}, {Wadsley}, \& {Quinn}}]{debattista_2006}
{Debattista}, V.~P., {Mayer}, L., {Carollo}, C.~M., {et~al.} 2006, \apj, 645, 209

\bibitem[{{D{\'\i}az-Garc{\'\i}a} {et~al.}(2016){D{\'\i}az-Garc{\'\i}a}, {Salo}, {Laurikainen}, \& {Herrera-Endoqui}}]{diaz-garcia_2016}
{D{\'\i}az-Garc{\'\i}a}, S., {Salo}, H., {Laurikainen}, E., \& {Herrera-Endoqui}, M. 2016, \aap, 587, A160

\bibitem[{{Ellison} {et~al.}(2011){Ellison}, {Nair}, {Patton}, {Scudder}, {Mendel}, \& {Simard}}]{ellison_2011}
{Ellison}, S.~L., {Nair}, P., {Patton}, D.~R., {et~al.} 2011, \mnras, 416, 2182

\bibitem[{{Elmegreen} \& {Elmegreen}(2005)}]{elmergreen_2005}
{Elmegreen}, B.~G., \& {Elmegreen}, D.~M. 2005, \apj, 627, 632

\bibitem[{{Erwin}(2019)}]{erwin_2019}
{Erwin}, P. 2019, \mnras, 489, 3553

\bibitem[{{Eskridge} {et~al.}(2000){Eskridge}, {Frogel}, {Pogge}, {Quillen}, {Davies}, {DePoy}, {Houdashelt}, {Kuchinski}, {Ram{\'\i}rez}, {Sellgren}, {Terndrup}, \& {Tiede}}]{eskridge_2000}
{Eskridge}, P.~B., {Frogel}, J.~A., {Pogge}, R.~W., {et~al.} 2000, \aj, 119, 536

\bibitem[{{F{\"o}rster Schreiber} {et~al.}(2011){F{\"o}rster Schreiber}, {Shapley}, {Genzel}, {Bouch{\'e}}, {Cresci}, {Davies}, {Erb}, {Genel}, {Lutz}, {Newman}, {Shapiro}, {Steidel}, {Sternberg}, \& {Tacconi}}]{foster_2011}
{F{\"o}rster Schreiber}, N.~M., {Shapley}, A.~E., {Genzel}, R., {et~al.} 2011, \apj, 739, 45

\bibitem[{{Fragkoudi} {et~al.}(2016){Fragkoudi}, {Athanassoula}, \& {Bosma}}]{fragkoudi_2016}
{Fragkoudi}, F., {Athanassoula}, E., \& {Bosma}, A. 2016, \mnras, 462, L41

\bibitem[{{Gadotti}(2009)}]{gadotti_2009}
{Gadotti}, D.~A. 2009, \mnras, 393, 1531

\bibitem[{{Gadotti} {et~al.}(2020){Gadotti}, {Bittner}, {Falc{\'o}n-Barroso}, {M{\'e}ndez-Abreu}, {Kim}, {Fragkoudi}, {de Lorenzo-C{\'a}ceres}, {Leaman}, {Neumann}, {Querejeta}, {S{\'a}nchez-Bl{\'a}zquez}, {Martig}, {Mart{\'\i}n-Navarro}, {P{\'e}rez}, {Seidel}, \& {van de Ven}}]{gadotti_2020}
{Gadotti}, D.~A., {Bittner}, A., {Falc{\'o}n-Barroso}, J., {et~al.} 2020, \aap, 643, A14

\bibitem[{{Galloway} {et~al.}(2015){Galloway}, {Willett}, {Fortson}, {Cardamone}, {Schawinski}, {Cheung}, {Lintott}, {Masters}, {Melvin}, \& {Simmons}}]{galloway_2015}
{Galloway}, M.~A., {Willett}, K.~W., {Fortson}, L.~F., {et~al.} 2015, \mnras, 448, 3442

\bibitem[{{Ghosh} {et~al.}(2024){Ghosh}, {Gadotti}, {Fragkoudi}, {Nagpal}, {Di Matteo}, \& {Cuomo}}]{ghosh_2024b}
{Ghosh}, S., {Gadotti}, D.~A., {Fragkoudi}, F., {et~al.} 2024, \mnras, 532, 4570

\bibitem[{{Ho} {et~al.}(1997){Ho}, {Filippenko}, \& {Sargent}}]{ho_1997}
{Ho}, L.~C., {Filippenko}, A.~V., \& {Sargent}, W. L.~W. 1997, \apjs, 112, 315

\bibitem[{{Hunt} \& {Malkan}(1999)}]{hunt_1999}
{Hunt}, L.~K., \& {Malkan}, M.~A. 1999, \apj, 516, 660

\bibitem[{{Inoue} \& {Saitoh}(2012)}]{inoue_2012}
{Inoue}, S., \& {Saitoh}, T.~R. 2012, \mnras, 422, 1902

\bibitem[{{Jacyszyn-Dobrzeniecka} {et~al.}(2016){Jacyszyn-Dobrzeniecka}, {Skowron}, {Mr{\'o}z}, {Skowron}, {Soszy{\'n}ski}, {Udalski}, {Pietrukowicz}, {Koz{\l}owski}, {Wyrzykowski}, {Poleski}, {Pawlak}, {Szyma{\'n}ski}, \& {Ulaczyk}}]{jacyszyn-Dobrzeniecka_2016}
{Jacyszyn-Dobrzeniecka}, A.~M., {Skowron}, D.~M., {Mr{\'o}z}, P., {et~al.} 2016, \actaa, 66, 149

\bibitem[{{James} \& {Percival}(2018)}]{james_2018}
{James}, P.~A., \& {Percival}, S.~M. 2018, \mnras, 474, 3101

\bibitem[{{Jogee} {et~al.}(2005){Jogee}, {Scoville}, \& {Kenney}}]{jogee_2005}
{Jogee}, S., {Scoville}, N., \& {Kenney}, J. D.~P. 2005, \apj, 630, 837

\bibitem[{{Kalita} {et~al.}(2025){Kalita}, {Silverman}, {Daddi}, {Mercier}, {Ho}, \& {Ding}}]{kalita_2025}
{Kalita}, B.~S., {Silverman}, J.~D., {Daddi}, E., {et~al.} 2025, \mnras, 537, 402

\bibitem[{{Kim} {et~al.}(2021){Kim}, {Athanassoula}, {Sheth}, {Bosma}, {Park}, {Lee}, \& {Ann}}]{kim_2021}
{Kim}, T., {Athanassoula}, E., {Sheth}, K., {et~al.} 2021, \apj, 922, 196

\bibitem[{{Kim} {et~al.}(2025){Kim}, {Gadotti}, {Park}, {Lee}, {Fragkoudi}, {Kim}, \& {Kim}}]{kim_2025b}
{Kim}, T., {Gadotti}, D.~A., {Park}, M.-g., {et~al.} 2025, \apj, 994, 105

\bibitem[{{Kim} {et~al.}(2012){Kim}, {Seo}, \& {Kim}}]{kim_2012}
{Kim}, W.-T., {Seo}, W.-Y., \& {Kim}, Y. 2012, \apj, 758, 14

\bibitem[{{Kormendy} \& {Fisher}(2005)}]{kormendy_2005}
{Kormendy}, J., \& {Fisher}, D.~B. 2005, in Revista Mexicana de Astronomia y Astrofisica Conference Series, Vol.~23, Revista Mexicana de Astronomia y Astrofisica Conference Series, ed. S.~{Torres-Peimbert} \& G.~{MacAlpine}, 101--108, \dodoi{10.48550/arXiv.astro-ph/0507525}

\bibitem[{{Kormendy} \& {Kennicutt}(2004)}]{kormendy_2004}
{Kormendy}, J., \& {Kennicutt}, Jr., R.~C. 2004, \araa, 42, 603

\bibitem[{{Kruk} {et~al.}(2017){Kruk}, {Lintott}, {Simmons}, {Bamford}, {Cardamone}, {Fortson}, {Hart}, {H{\"a}u{\ss}ler}, {Masters}, {Nichol}, {Schawinski}, \& {Smethurst}}]{kruk_2017}
{Kruk}, S.~J., {Lintott}, C.~J., {Simmons}, B.~D., {et~al.} 2017, \mnras, 469, 3363

\bibitem[{{Kuno} {et~al.}(2007){Kuno}, {Sato}, {Nakanishi}, {Hirota}, {Tosaki}, {Shioya}, {Sorai}, {Nakai}, {Nishiyama}, \& {Vila-Vilar{\'o}}}]{kuno_2007}
{Kuno}, N., {Sato}, N., {Nakanishi}, H., {et~al.} 2007, \pasj, 59, 117

\bibitem[{{Laurikainen} \& {Salo}(2002)}]{laurikainen_2002}
{Laurikainen}, E., \& {Salo}, H. 2002, \mnras, 337, 1118

\bibitem[{{Lee} {et~al.}(2012){Lee}, {Woo}, {Lee}, {Hwang}, {Lee}, {Sohn}, \& {Lee}}]{lee_2012}
{Lee}, G.-H., {Woo}, J.-H., {Lee}, M.~G., {et~al.} 2012, \apj, 750, 141

\bibitem[{{Lee} {et~al.}(2020){Lee}, {Park}, {Ann}, {Kim}, \& {Seo}}]{lee_2020}
{Lee}, Y.~H., {Park}, M.-G., {Ann}, H.~B., {Kim}, T., \& {Seo}, W.-Y. 2020, \apj, 899, 84

\bibitem[{{{\L}okas}(2021)}]{lokas_2021}
{{\L}okas}, E.~L. 2021, \aap, 655, A97

\bibitem[{{Martinez-Valpuesta} \& {Shlosman}(2004)}]{martinez_2004}
{Martinez-Valpuesta}, I., \& {Shlosman}, I. 2004, \apjl, 613, L29

\bibitem[{{Masters} {et~al.}(2011){Masters}, {Nichol}, {Hoyle}, {Lintott}, {Bamford}, {Edmondson}, {Fortson}, {Keel}, {Schawinski}, {Smith}, \& {Thomas}}]{masters_2011}
{Masters}, K.~L., {Nichol}, R.~C., {Hoyle}, B., {et~al.} 2011, \mnras, 411, 2026

\bibitem[{{Men{\'e}ndez-Delmestre} {et~al.}(2007){Men{\'e}ndez-Delmestre}, {Sheth}, {Schinnerer}, {Jarrett}, \& {Scoville}}]{menedez_2007}
{Men{\'e}ndez-Delmestre}, K., {Sheth}, K., {Schinnerer}, E., {Jarrett}, T.~H., \& {Scoville}, N.~Z. 2007, \apj, 657, 790

\bibitem[{{Nelson} {et~al.}(2019){Nelson}, {Pillepich}, {Springel}, {Pakmor}, {Weinberger}, {Genel}, {Torrey}, {Vogelsberger}, {Marinacci}, \& {Hernquist}}]{nelson_2019}
{Nelson}, D., {Pillepich}, A., {Springel}, V., {et~al.} 2019, \mnras, 490, 3234

\bibitem[{{Newnham} {et~al.}(2020){Newnham}, {Hess}, {Masters}, {Kruk}, {Penny}, {Lingard}, \& {Smethurst}}]{newnham_2020}
{Newnham}, L., {Hess}, K.~M., {Masters}, K.~L., {et~al.} 2020, \mnras, 492, 4697

\bibitem[{{Odewahn}(1996)}]{odewahn_1996}
{Odewahn}, S.~C. 1996, Astronomical Society of the Pacific Conference Series, 106, 139

\bibitem[{{Oh} {et~al.}(2012){Oh}, {Oh}, \& {Yi}}]{oh_2012}
{Oh}, S., {Oh}, K., \& {Yi}, S.~K. 2012, \apjs, 198, 4

\bibitem[{{Ohta} {et~al.}(1990){Ohta}, {Hamabe}, \& {Wakamatsu}}]{ohta_1990}
{Ohta}, K., {Hamabe}, M., \& {Wakamatsu}, K.-I. 1990, \apj, 357, 71

\bibitem[{{Pardy} {et~al.}(2016){Pardy}, {D'Onghia}, {Athanassoula}, {Wilcots}, \& {Sheth}}]{pardy_2016}
{Pardy}, S.~A., {D'Onghia}, E., {Athanassoula}, E., {Wilcots}, E.~M., \& {Sheth}, K. 2016, \apj, 827, 149

\bibitem[{{Patra} \& {Jog}(2019)}]{patra_2019}
{Patra}, N.~N., \& {Jog}, C.~J. 2019, \mnras, 488, 4942

\bibitem[{{Peschken} \& {{\L}okas}(2019)}]{Peschken2019}
{Peschken}, N., \& {{\L}okas}, E.~L. 2019, \mnras, 483, 2721

\bibitem[{{Pillepich} {et~al.}(2018){Pillepich}, {Springel}, {Nelson}, {Genel}, {Naiman}, {Pakmor}, {Hernquist}, {Torrey}, {Vogelsberger}, {Weinberger}, \& {Marinacci}}]{Pillepich2018}
{Pillepich}, A., {Springel}, V., {Nelson}, D., {et~al.} 2018, \mnras, 473, 4077

\bibitem[{{Pillepich} {et~al.}(2019){Pillepich}, {Nelson}, {Springel}, {Pakmor}, {Torrey}, {Weinberger}, {Vogelsberger}, {Marinacci}, {Genel}, {van der Wel}, \& {Hernquist}}]{pillepich_2019}
{Pillepich}, A., {Nelson}, D., {Springel}, V., {et~al.} 2019, \mnras, 490, 3196

\bibitem[{{Planck Collaboration} {et~al.}(2016){Planck Collaboration}, {Ade}, {Aghanim}, {Arnaud}, {Ashdown}, {Aumont}, {Baccigalupi}, {Banday}, {Barreiro}, {Bartlett}, {Bartolo}, {Battaner}, {Battye}, {Benabed}, {Beno{\^\i}t}, {Benoit-L{\'e}vy}, {Bernard}, {Bersanelli}, {Bielewicz}, {Bock}, {Bonaldi}, {Bonavera}, {Bond}, {Borrill}, {Bouchet}, {Boulanger}, {Bucher}, {Burigana}, {Butler}, {Calabrese}, {Cardoso}, {Catalano}, {Challinor}, {Chamballu}, {Chary}, {Chiang}, {Chluba}, {Christensen}, {Church}, {Clements}, {Colombi}, {Colombo}, {Combet}, {Coulais}, {Crill}, {Curto}, {Cuttaia}, {Danese}, {Davies}, {Davis}, {de Bernardis}, {de Rosa}, {de Zotti}, {Delabrouille}, {D{\'e}sert}, {Di Valentino}, {Dickinson}, {Diego}, {Dolag}, {Dole}, {Donzelli}, {Dor{\'e}}, {Douspis}, {Ducout}, {Dunkley}, {Dupac}, {Efstathiou}, {Elsner}, {En{\ss}lin}, {Eriksen}, {Farhang}, {Fergusson}, {Finelli}, {Forni}, {Frailis}, {Fraisse}, {Franceschi}, {Frejsel}, {Galeotta}, {Galli}, {Ganga}, {Gauthier}, {Gerbino}, {Ghosh}, {Giard},
  {Giraud-H{\'e}raud}, {Giusarma}, {Gjerl{\o}w}, {Gonz{\'a}lez-Nuevo}, {G{\'o}rski}, {Gratton}, {Gregorio}, {Gruppuso}, {Gudmundsson}, {Hamann}, {Hansen}, {Hanson}, {Harrison}, {Helou}, {Henrot-Versill{\'e}}, {Hern{\'a}ndez-Monteagudo}, {Herranz}, {Hildebrandt}, {Hivon}, {Hobson}, {Holmes}, {Hornstrup}, {Hovest}, {Huang}, {Huffenberger}, {Hurier}, {Jaffe}, {Jaffe}, {Jones}, {Juvela}, {Keih{\"a}nen}, {Keskitalo}, {Kisner}, {Kneissl}, {Knoche}, {Knox}, {Kunz}, {Kurki-Suonio}, {Lagache}, {L{\"a}hteenm{\"a}ki}, {Lamarre}, {Lasenby}, {Lattanzi}, {Lawrence}, {Leahy}, {Leonardi}, {Lesgourgues}, {Levrier}, {Lewis}, {Liguori}, {Lilje}, {Linden-V{\o}rnle}, {L{\'o}pez-Caniego}, {Lubin}, {Mac{\'\i}as-P{\'e}rez}, {Maggio}, {Maino}, {Mandolesi}, {Mangilli}, {Marchini}, {Maris}, {Martin}, {Martinelli}, {Mart{\'\i}nez-Gonz{\'a}lez}, {Masi}, {Matarrese}, {McGehee}, {Meinhold}, {Melchiorri}, {Melin}, {Mendes}, {Mennella}, {Migliaccio}, {Millea}, {Mitra}, {Miville-Desch{\^e}nes}, {Moneti}, {Montier}, {Morgante}, {Mortlock},
  {Moss}, {Munshi}, {Murphy}, {Naselsky}, {Nati}, {Natoli}, {Netterfield}, {N{\o}rgaard-Nielsen}, {Noviello}, {Novikov}, {Novikov}, {Oxborrow}, {Paci}, {Pagano}, {Pajot}, {Paladini}, {Paoletti}, {Partridge}, {Pasian}, {Patanchon}, {Pearson}, {Perdereau}, {Perotto}, {Perrotta}, {Pettorino}, {Piacentini}, {Piat}, {Pierpaoli}, {Pietrobon}, {Plaszczynski}, {Pointecouteau}, {Polenta}, {Popa}, {Pratt}, \& {Pr{\'e}zeau}}]{planck_2016}
{Planck Collaboration}, {Ade}, P.~A.~R., {Aghanim}, N., {et~al.} 2016, \aap, 594, A13

\bibitem[{{Raha} {et~al.}(1991){Raha}, {Sellwood}, {James}, \& {Kahn}}]{raha_1991}
{Raha}, N., {Sellwood}, J.~A., {James}, R.~A., \& {Kahn}, F.~D. 1991, \nat, 352, 411

\bibitem[{{Renzini} \& {Peng}(2015)}]{renzini_2015}
{Renzini}, A., \& {Peng}, Y.-j. 2015, \apjl, 801, L29

\bibitem[{{Rosas-Guevara} {et~al.}(2020){Rosas-Guevara}, {Bonoli}, {Dotti}, {Zana}, {Nelson}, {Pillepich}, {Ho}, {Izquierdo-Villalba}, {Hernquist}, \& {Pakmor}}]{RosasGuevara2020}
{Rosas-Guevara}, Y., {Bonoli}, S., {Dotti}, M., {et~al.} 2020, \mnras, 491, 2547

\bibitem[{{Rosas-Guevara} {et~al.}(2022){Rosas-Guevara}, {Bonoli}, {Dotti}, {Izquierdo-Villalba}, {Lupi}, {Zana}, {Bonetti}, {Nelson}, {Springel}, {Hernquist}, \& {Vogelsberger}}]{RosasGuevara2022}
{Rosas-Guevara}, Y., {Bonoli}, S., {Dotti}, M., {et~al.} 2022, \mnras, 512, 5339

\bibitem[{{Sakamoto} {et~al.}(1999){Sakamoto}, {Okumura}, {Ishizuki}, \& {Scoville}}]{sakamoto_1999}
{Sakamoto}, K., {Okumura}, S.~K., {Ishizuki}, S., \& {Scoville}, N.~Z. 1999, \apj, 525, 691

\bibitem[{{Salo} {et~al.}(2010){Salo}, {Laurikainen}, {Buta}, \& {Knapen}}]{salo_2010}
{Salo}, H., {Laurikainen}, E., {Buta}, R., \& {Knapen}, J.~H. 2010, \apjl, 715, L56

\bibitem[{{S{\'a}nchez-Mart{\'\i}n} {et~al.}(2023){S{\'a}nchez-Mart{\'\i}n}, {Garc{\'\i}a-G{\'o}mez}, {Masdemont}, \& {Romero-G{\'o}mez}}]{sanchezmartin_2023}
{S{\'a}nchez-Mart{\'\i}n}, P., {Garc{\'\i}a-G{\'o}mez}, C., {Masdemont}, J.~J., \& {Romero-G{\'o}mez}, M. 2023, \mnras, 520, 3909

\bibitem[{{Sellwood} \& {Wilkinson}(1993)}]{sellwood_1993}
{Sellwood}, J.~A., \& {Wilkinson}, A. 1993, Reports on Progress in Physics, 56, 173

\bibitem[{{Semczuk} {et~al.}(2024){Semczuk}, {Dehnen}, {Sch{\"o}nrich}, \& {Athanassoula}}]{semczuk_2024}
{Semczuk}, M., {Dehnen}, W., {Sch{\"o}nrich}, R., \& {Athanassoula}, E. 2024, \aap, 692, A159

\bibitem[{{Seo} {et~al.}(2019){Seo}, {Kim}, {Kwak}, {Hsieh}, {Han}, \& {Hopkins}}]{seo_2019}
{Seo}, W.-Y., {Kim}, W.-T., {Kwak}, S., {et~al.} 2019, \apj, 872, 5

\bibitem[{{Sheth} {et~al.}(2000){Sheth}, {Regan}, {Vogel}, \& {Teuben}}]{sheth_2000}
{Sheth}, K., {Regan}, M.~W., {Vogel}, S.~N., \& {Teuben}, P.~J. 2000, \apj, 532, 221

\bibitem[{{Sheth} {et~al.}(2005){Sheth}, {Vogel}, {Regan}, {Thornley}, \& {Teuben}}]{sheth_2005}
{Sheth}, K., {Vogel}, S.~N., {Regan}, M.~W., {Thornley}, M.~D., \& {Teuben}, P.~J. 2005, \apj, 632, 217

\bibitem[{{Sheth} {et~al.}(2008){Sheth}, {Elmegreen}, {Elmegreen}, {Capak}, {Abraham}, {Athanassoula}, {Ellis}, {Mobasher}, {Salvato}, {Schinnerer}, {Scoville}, {Spalsbury}, {Strubbe}, {Carollo}, {Rich}, \& {West}}]{sheth_2008}
{Sheth}, K., {Elmegreen}, D.~M., {Elmegreen}, B.~G., {et~al.} 2008, \apj, 675, 1141

\bibitem[{{Shlosman}(1994)}]{combes_1994}
{Shlosman}, I., ed. 1994, {Mass-transfer induced activity in galaxies}

\bibitem[{{Simkin} {et~al.}(1980){Simkin}, {Su}, \& {Schwarz}}]{simkin_1980}
{Simkin}, S.~M., {Su}, H.~J., \& {Schwarz}, M.~P. 1980, \apj, 237, 404

\bibitem[{{Sormani} {et~al.}(2015){Sormani}, {Binney}, \& {Magorrian}}]{sormani_2015}
{Sormani}, M.~C., {Binney}, J., \& {Magorrian}, J. 2015, \mnras, 449, 2421

\bibitem[{{van de Ven} \& {Fathi}(2010)}]{vandeven_2010ApJ...723..767V}
{van de Ven}, G., \& {Fathi}, K. 2010, \apj, 723, 767

\bibitem[{{van der Marel} \& {Cioni}(2001)}]{vandermarel_2001}
{van der Marel}, R.~P., \& {Cioni}, M.-R.~L. 2001, \aj, 122, 1807

\bibitem[{{Wang} \& {Zhou}(2025)}]{wang_2025}
{Wang}, W., \& {Zhou}, Z. 2025, \apj, 982, 129

\bibitem[{{Waters} {et~al.}(2024){Waters}, {Peterson}, {Emami}, {Shen}, {Hernquist}, {Smith}, {Vogelsberger}, {Alcock}, {Tremblay}, {Liska}, {Forbes}, \& {Moreno}}]{waters_2024}
{Waters}, T.~K., {Peterson}, C., {Emami}, R., {et~al.} 2024, \apj, 961, 193

\bibitem[{{Yu} {et~al.}(2018){Yu}, {Ho}, {Barth}, \& {Li}}]{yu_2018}
{Yu}, S.-Y., {Ho}, L.~C., {Barth}, A.~J., \& {Li}, Z.-Y. 2018, \apj, 862, 13

\bibitem[{{Zana} {et~al.}(2022){Zana}, {Lupi}, {Bonetti}, {Dotti}, {Rosas-Guevara}, {Izquierdo-Villalba}, {Bonoli}, {Hernquist}, \& {Nelson}}]{zana_2022}
{Zana}, T., {Lupi}, A., {Bonetti}, M., {et~al.} 2022, \mnras, 515, 1524

\bibitem[{{Zee} {et~al.}(2023){Zee}, {Paudel}, {Moon}, \& {Yoon}}]{zee_2023}
{Zee}, W.-B.~G., {Paudel}, S., {Moon}, J.-S., \& {Yoon}, S.-J. 2023, \apj, 949, 91

\bibitem[{{Zhao} {et~al.}(2020){Zhao}, {Du}, {Ho}, {Debattista}, \& {Shi}}]{Zhao2020}
{Zhao}, D., {Du}, M., {Ho}, L.~C., {Debattista}, V.~P., \& {Shi}, J. 2020, \apj, 904, 170

\bibitem[{{Zhou} {et~al.}(2020){Zhou}, {Zhu}, {Wang}, \& {Feng}}]{zhou_2020}
{Zhou}, Z.-B., {Zhu}, W., {Wang}, Y., \& {Feng}, L.-L. 2020, \apj, 895, 92

\end{thebibliography}

